An Algorithmic Classification of Generalized Pseudo-Anosov Homeomorphisms via Geometric Markov Partitions

This thesis provides a classification of generalized pseudo-Anosov homeomorphisms up to topological conjugacy using an algorithmic approach. A Markov partition of a generalized pseudo-Anosov homeomorphism is a decomposition of the surface into a finite number of rectangles with disjoint interiors, such that their images intersect with any other rectangle in the Markov partition along a finite number of horizontal sub-rectangles. Every generalized pseudo-Anosov homeomorphism has a Markov partition, and, by using the surface's orientation, we can endow any Markov partition with a geometrization. The geometric type of a geometric Markov partition was defined by Bonatti and Langevin in their book, "Diffeomorphismes de Smale des surfaces", to classify saddle-type basic pieces for structurally stable diffeomorphisms on surfaces. A geometric type is an abstract combinatorial object that generalizes the incidence matrix of a Markov partition. It takes into account not only the number of times the image of a rectangle intersects with any other rectangle in the family but also the order and change of orientation induced by the homeomorphisms. This thesis employs the geometric type of a geometric Markov partition to classify conjugacy classes of pseudo-Anosov homeomorphisms. The classification is provided by the three main results in this manuscript: I) The geometric type is a complete invariant of conjugation. II) A criterion is provided for determining whether an abstract geometric type is realized by a geometric Markov partition of a pseudo-Anosov homeomorphism. III) An algorithm is described for determining whether two geometric types in the pseudo-Anosov class are realized by generalized pseudo-Anosov homeomorphisms that are topologically conjugated or not.

==> ExistenceCanonic/Canonical.tex <==
\section{Construction of Markov partition and the primitive family}\label{Section: Canonical}



%%%%%The recipe

\begin{prop}\label{Prop: A recipy for Markov partitions}
A recipe for Markov partitions
\end{prop}

%%%%%First intesection points

\begin{defi}\label{Defi: first intersection points}
	content...
\end{defi}


\begin{lemm}\label{Lemm: Finite number first intersection points}
	content...
\end{lemm}


 

\begin{theo}\label{Theo: Conjugates then primitive Markov partition}
	Let $f$ and $g$ be conjugated pseudo-Anosov maps, and $h$ a homeomorphism which conjugate them, $h\circ f \circ h^{-1} = g$. Let $z$ first intersection point of $f$, then
	\begin{itemize}
	\item $h(z)$ is a first intersection point of $z$
	\item $n(f)=n(g)$ 
	\item for all $p\geq n(f),n(g)$,  $h(\cR(p,z))=\cR(p,h(z))$ is a Markov partition for $g$.
	\item Under  the $h$-induced \emph{geometrization} of  $\cR(p,h(z))$, $\cR(p,h(z))$ and $\cR(p,z)$ have the same geometric type.
	\end{itemize}
\end{theo}



\begin{theo}\ref{Theo: Finite orbits of primitive Markov partitions}
	For every $p>n(f)$ there exist a finite but non-empty set of orbits of primitive adapted Markov partitions.\\
	The set of primitive Markov partition of order $p$ is denoted $\cM(f,p)$
\end{theo}


==> ExistenceCanonic/Secgenus.tex <==
\section{From a geometric type to the genus of the surface}


\begin{prop}\label{Prop: Algoritm for genus}
	Let $T$ a geometric type in the pseudo-Anosov class and be $(\Sigma_T,\sigma_T)$ its canonical combinatorial model. There is an algorithm for every one of the following problems.
	\begin{itemize}
		\item Determine the codes which correspond to boundary periodic codes.
		\item Determine if a boundary periodic point is or not in the boundary of $\Sigma_T$;
		\item Given a periodic boundary code give back the number of $k$-prong it have. In particular it distinguishes  Spine-type singularities and $k$-prongs.
		\item To calculate the genus of $\Sigma_T$ and the number of boundary components.
	\end{itemize}
\end{prop}


==> Preliminares/Algofinitegenus.tex <==
\subsection{Algorithmic Determination of Finite Genus and Impasse }\label{Sub-sec: algoritm finite genus}


The objective is to prove the following proposition that will serve as the key element in determining, algorithmically and in finite time, whether a geometric type belongs to the pseudo-Anosov class or not. In the future, we will derive the property of double boundaries from the fact that the incidence matrix of a geometric type in the pseudo-Anosov class is mixing. Therefore, we formulate this property as the first one to be verified.

\begin{prop}\label{Prop: mixing+genus+impase is algorithm}
	Given any abstract geometric type $T=(n\{(h_i,v_i),\},\Phi)$, there exists a finite algorithm that can determine whether $T$ satisfies the following properties:
	\begin{enumerate}
		\item The incidence matrix of $T$, $A(T)$ is mixing. 
		\item The genus of $T$ is finite.
		\item  $T$ exhibits an impasse.
	\end{enumerate}
Furthermore, the number of iterations of $T$ required by the algorithm to determine these properties is upper bounded by $6n$, where $n$ represents the size of $T$.
\end{prop}



\begin{proof}

We have formulated specific conditions on the combinatorics of $T$ to determine whether $T^n$ has an impasse or one of the three obstructions to have finite genus. Furthermore, according to Theorem \ref{Theo: finite type iff non-obstruction}, determining whether or not $T$ has finite genus requires computing at most $T^{6n}$. To determine whether $T$ has an impasse, Theorem \ref{Theo: Geometric and combinatoric are equivalent} states that it is necessary to compute at most $T^{2n+1}$. Since $n\geq1$, it is clear that $2n+1<6n$, which provides the upper bound we claim in the proposition. Proposition \ref{Prop: algorithm iterations type} asserts that the computation of $T^{6n}$ is algorithmic, thus confirming the existence of an algorithm to determine the finite genus and the presence of an impasse for $T$.




We have left the mixing criterion for last. The following lemma is the basis for the upper bound on the number of iterations to verify the mixing of the incidence matrix.

\begin{prop}\label{Prop: bound positive incidence matriz }
If $A$ is a non-negative mixing matrix of size $n \times n$, then $A^n$ is positive definite.
\end{prop}

\begin{proof}
	
	Consider the directed graph $\mathcal{G}$ with $n$ vertices corresponding to the matrix $A$. In this graph, there is an edge pointing from vertex $v_i$ to vertex $v_j$ if and only if $a_{ij} > 0$ in the matrix $A$. Since $A$ is mixing, it means that there is always a path from any vertex $v_i$ to any other vertex $v_j$ in the graph $\mathcal{G}$.
	
		To prove our Lemma, it is sufficient to demonstrate that there exists a path of length less than or equal to $n$ between any two vertices in the graph.
	

	
	Consider a path $\gamma = [v_{i(1)}, \cdots, v_{i(m)}]$ from $v_i = v_{i(1)}$ to $v_j = v_{i(m)}$ in the graph $\mathcal{G}$. Let $\gamma$ have $m$ vertices and be of minimum length among all paths connecting these vertices.
	
	If any two vertices of the path $\gamma$ are equal, it implies the existence of a cycle within $\gamma$. We can eliminate this cycle and obtain a new path $\gamma'$ from $v_i$ to $v_j$ with a shorter length than $\gamma$. This contradicts the assumption that $\gamma$ has the minimum length. Hence, all vertices in $\gamma$ must be distinct.
	
	Therefore, the length of $\gamma$ is necessarily less than or equal to $n$, since there are only $n$ distinct vertices in the graph.
\end{proof}


If $T$ is in the pseudo-Anosov class, we have $A^n(T) = A(T^n)$. According to the previous Lemma, if $A(T)$ is a non-negative matrix, then $A(T^n)$ is positive definite. This implies that $A(T^n)$ is mixing and does not have double boundaries. Therefore, for a given geometric type $T$ with $A(T)$ being a non-negative matrix, the positivity of $A(T^n)$ is equivalent to its mixing property, which in turn implies the absence of double boundaries.

\begin{coro}\label{Coro: algoritmic mixing}
Given a geometric type $T$, if $A(T^n)$ is not positive definite, then $T$ is not in the pseudo-Anosov class.
\end{coro}

Clearly, we only need to iterate $T$ $n$ times, and the upper bound given in the proposition remains valid. 
This concludes our proof.
\end{proof}

==> Realization/Algortmicgenimpasse.tex <==
\subsection{ Combinatorial formulation of finite genus and impasse}\label{Sub-sec: Comb Impasse genus}


The obstructions described above provide a valuable tool for analyzing our Markov partition from a visual perspective. However, in order to obtain an algorithmic characterization of the pseudo-Anosov class of geometric types, we need to translate these three topological obstructions and the impasse condition into a combinatorial formulation that allows us to determine in finite time whether or not these conditions are satisfied.

The key insight lies in Proposition \ref{Prop: properties ribbons}, where we observed that every ribbon of $k$-generation corresponds to the image of a horizontal strip between two consecutive horizontal sub-rectangles of the Markov partition for the map $\phi^k$ under the projection $\pi$. In this section, we will consider the geometric type.


$$
T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi_T:=(\rho_T,\epsilon_T )).
$$


The trick in our upcoming definitions is that whenever we want to talk about a "ribbon" with a certain property, we need to refer to two consecutive horizontal rectangles and analyze their images under $\phi^k$. This way, a "ribbon" is formed, and we can express the obstructions and the impasse property in terms of the images of these consecutive horizontal rectangles.

\subsubsection{Combinatorial obstructions for finite genus.}
\begin{defi}\label{Defi: Type 1 combinatoric}
	A geometric type $T$ satisfies the \emph{combinatorial condition} of type-$(1)$ if and only if there are:
	
	\begin{itemize}
		\item Three (not necessarily distinct) numbers, $k,i_0,i_1\in \{1,\cdots,n\}$.
		\item Three different  numbers, $l_0,l_1,l_2\in \{1,\cdots,v_{k}\}$ with $l_0<l_1<l_2$.
		\item A pair  $(k',l')\in\cV(T)$, such that $(k',l')\notin \{(k,l):l_0\leq l \leq l_2\}$.
		\item And four pairs, $(i_0,j_0),(i_0,j_0+1),(i_1,j_1)(i_1,j_1+1)\in \cH(T)$
		\end{itemize}
	Such that they satisfy one of the following relations:
\begin{enumerate}
\item If  $\rho_T(i_0,j_0)=(k,l_0)$ and $\rho_T(i_0,j_0+1)=(k,l_2)$, we have two available possibilities:
\begin{itemize}
	\item[i)] $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$.  In such a case:
	 $$
	 \rho_T(i_1,j_1)=(k,l_1), \, \epsilon_T(i_1,j_1)=1 \text{ and } \rho_T(i_1,j_1+1)=(k',l'),
	 $$
	  or well,
	  $$
	  \rho_T(i_1,j_1+1)=(k,l_1), \,  \epsilon_T(i_1,j_1+1)=-1,  \text{ and } \rho_T(i_1,j_1)=(k',l').
	  $$
	
	\item[ii)] $\epsilon_T(i_0,j_0)=-1$ and $\epsilon_T(i_0,j_0+1)=1$. In such a case  
	$$
	\rho_T(i_1,j_1)=(k,l_1), \,  \epsilon_T(i_1,j_1)=-1 \text{ and  }\rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
	\rho_T(i_1,j_1+1)=(k,l_1), \,  \epsilon_T(i_1,j_1)=1 \text{ and  } \rho_T(i_1,j_1)=(k',l').
	$$.
	
	
\end{itemize}
\item  In the symmetric case when, $\rho_T(i_0,j_0)=(k,l_2)$ and $\rho_T(i_0,j_0+1)=(k,l_0)$ there are two options:
\begin{itemize}
	\item[i)] $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$. In such a case: 
	$$
	\rho_T(i_1,j_1)=(k,l_1), \, \epsilon_T(i_1,j_1)=1  \text{ and }  \rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
	\rho_T(i_1,j_1+1)=(k,l_1), \, \epsilon_T(i_1,j_1+1)=-1  \text{ and }  \rho_T(i_1,j_1)=(k',l')
	$$

	\item[ii)]  $\epsilon_T(i_0,j_0)=-1$ and $\epsilon_T(i_0,j_0+1)=1$. In such a case:  
	$$
	\rho_T(i_1,j_1)=(k,l_1),\, \epsilon_T(i_1,j_1)=-1 \text{ and  } \rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
\rho_T(i_1,j_1+1)=(k,l_1),\, \epsilon_T(i_1,j_1)=1 \text{ and  } 	\rho_T(i_1,j_1)=(k',l').
	$$
\end{itemize}
\end{enumerate}
	A geometric type has the \emph{combinatorial obstruction} of type-$(1)$ if there exists $m \in \mathbb{N}_{>0}$ such that $T^m$ satisfies the combinatorial condition of type-$(1)$.
\end{defi}


The way we have defined the combinatorial condition of type $(1)$ is by identifying the $1$-generation ribbons of the Markov partition $\cR_0$ in $\cR_1$ that give rise to the topological obstruction of type-$(1)$ in $\cR_1$ as the image of a horizontal stripe contained between two consecutive sub-rectangles. This understanding of ribbons corresponds to two consecutive elements $(i,j)$ and $(i,j+1)$ in $\cH$ and their images under $\rho_T$ in $\cV$, which represent the ribbons. In the following lemma we are going to follow the Figure \ref{Fig: Type one proof} to explain or proof. 


\begin{figure}[h]
	\centering
	\includegraphics[width=0.83\textwidth]{Preliminares/Imagenes/type1proof.png}
	\caption{Type $(1)$ combinatorial condition}
	\label{Fig: Type one proof}
\end{figure}



\begin{lemm}\label{Lemm: Equiv com and top type 1}
A geometric type $T$ has the combinatorial condition of type-$(1)$ if and only if the Markov partition in $\cR_1$ exhibits the topological obstruction of type-$(1)$.
\end{lemm}


\begin{proof}
The terms $(k,l_0)$, $(k,l_1)$, and $(k,l_2)$ represent three different vertical sub-rectangles of $R_k$ ordered by the horizontal orientation of $R_k$. The term $(k',l')$ represents a horizontal sub-rectangle of $\cR$ that is not located between the rectangles $V^k_{l_0}$ and $V^k_{l_2}$. Let's illustrate the meaning of the condition in the first case, as the rest are symmetric.

The conditions $\rho(i_0,j_0)=(k,l_0)$ and $\rho(i_0,j_0+1)=(k,l_2)$ are equivalent to the fact that the image under $f$ of the horizontal strip $\underline{H}_{j_0}$ bounded by $H^{i_0}_{j_0}$ and $H^{i_0}_{j_0+1}$ is a ribbon $r=f(\underline{H}_{j_0})$ of the first generation that connects the horizontal boundaries of $V^k_{l_0}$ and $V^{k}_{l_2}$. In this case, in Item $(i)$, the conditions $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$ means that the ribbon $r$ connects the upper boundary of $V^k_{l_0}$ with the upper boundary of $V^{k}_{l_2}$.

The conditions $\rho(i_1,j_1)=(k,l_1)$ and $\rho(i_1,j_1+1)=(k',l')$ indicate that the image of the strip $\underline{H}_{j_1}$ bounded by $H^{i_1}_{j_1}$ and  $H^{i_1}_{j_1+1}$ is a ribbon $r'$ connecting a horizontal boundary of $V^k_{l_1}$ with a horizontal boundary of $V^{k'}_{l'}$. Moreover, since $\epsilon_T(i_1,j_1)=1$, it means that $r'$ connects the upper boundary of $V^k_{l_1}$ with the stable boundary $\alpha$ of $V^{k'}{l'}$. But the condition $(k',l')\notin \{(k,l): l_0\leq l\leq l_2\}$ ensures that the stable boundary $\alpha$ cannot be situated between the upper boundaries of $V^k{l_0}$ and $V^k_{l_2}$, as we have specified from the beginning. Therefore the Markov partition $\cR_1$ have the topological obstruction of type $(1)$.

Is not difficult to see that if $\cR_1$ have the topological obstruction of type $(1)$, then the ribbons $r$ and $r'$ given by the definition \ref{Defi: Type 1 obstruction top}, are determined by be the image of a stripe comprised between consecutive sub-rectangles $H^{i_0}_{j_0}$ and $H^{i_0}_{j_0}$ for $r$ and $H^{i_1}_{j_1}$ and $H^{i_1}_{j_1+1}$ for $r'$. The rest of the conditions are totally determined.
\end{proof}





This coding method of representing a ribbon as two consecutive indices $(i,j)$ and $(i,j+1)$ in $\cH$ will be utilized frequently throughout this subsection. 


\begin{defi}\label{Defi: Type 2 combinatoric}
	The geometric type $T$ has the type-$(2)$ \emph{combinatorial condition} if and only if there are:
	\begin{itemize}
\item Four different pairs $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)\in \cV(T)$ with $l_1<l_2$ and $l^1<l^2$.
\item For pair $(i_1,j_1),(i_1,j_1+1),(i_2,j_2),(i_2,j_2+1)\in \cH(T)$ 
	\end{itemize}
Such that:
	$$
	\rho_T(i_1,j_1)=(k_1,l^1) \text{ and } \rho_T(i_1,j^1+1)=(k_2,l_2).
	$$
	
Additionally, depending on the signs of $\epsilon_T(i_1,j_1)$ and $\epsilon_T(i_1,j_1+1)$ we have the next constrictions:
	
	\begin{enumerate}
\item If $\epsilon_T(i_1,j_1)=\epsilon_T(i_1,j_1+1)$, then we have two options:
\begin{itemize}
\item[i)] If $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ then: $$\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)$$.

\item[ii)] If  $\rho_T(i_2,j_2)= (k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$. Then
$$-\epsilon_T(i_1,j_1)=-\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)$$.
\end{itemize}

\item If $\epsilon_T(i_1,j_1)=-\epsilon_T(i_1,j_1+1)$, then we have two options:

\begin{itemize}
\item[i)] If $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ then:
$$
\epsilon_T(i_2,j_2)=\epsilon_T(i_1,j_1) \text{ and  } \epsilon_T(i_2,j_2+1)=\epsilon_T(i_1,j_1+1).
$$
\item[ii)] If $\rho_T(i_2,j_2)=(k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$ then:
$$
\epsilon_T(i_2,j_2)=-\epsilon_T(i_1,j_1+1) \text{ and  } \epsilon_T(i_2,j_2+1)=-\epsilon_T(i_1,j_1).
$$

\end{itemize}

\end{enumerate}

\begin{comment}

$l'_1\in \{1,\cdots,l_1-1,l_1+1, v_{k+1}\}$ and $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ such that,  $l'_1<l_1$ if and only if  $l'_2>l_2$ and there are two options
$$
\Phi(i_2,j_2)=(k_1,l'_1,\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l'_2,\epsilon(i_2,j_2+2)) 
$$
or well
$$
\Phi(i_2,j_2)=(k_2,l'_2\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_1,l'_1,\epsilon(i_2,j_2+2)).
$$

\item Suppose $\epsilon(i_1,j_1)=-\epsilon(i_2,j_2+1)$. Then there are $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ and $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ such that, $l'_1<l_1$ if and only if $l'_2<l_2$ and in this situation two possibilities are admissible:
$$
\Phi(i_2,j_2)=(k_1,l'_1,\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l'_2,\epsilon(i_2,j_2+2)) 
$$
or well
$$
\Phi(i_2,j_2)=(k_2,l'_2\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_1,l'_1,\epsilon(i_2,j_2+2)).
$$
\end{itemize}
\end{comment}


A geometric type $T$ has the \emph{combinatorial obstruction} of type-$(2)$ if there exists $m\in \NN$ such that $T^m$ satisfies the combinatorial condition of type-$(2)$.
\end{defi}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.83\textwidth]{Preliminares/Imagenes/tipp2pof.png}
	\caption{Type $(2)$ combinatorial condition}
	\label{Fig: Type two proof}
\end{figure}


 The Figure \ref{Fig: Type two proof} give some help to understand the proof.
 
\begin{lemm}\label{Lemm: Equiv com and top type 2} 
A geometric type $T$ satisfies the combinatorial condition of type-$(2)$ if and only if the Markov partition $\cR_0$ has the topological obstruction of type-$(2)$ on $\cR_1$.
\end{lemm}


\begin{proof}
The pairs $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)$ represent the respective vertical sub-rectangles of $\cR$ and the condition $\rho_T(i_1,j_1)=(k_1,l^1) \text{ and } \rho_T(i_1,j^1+1)=(k_2,l_2)$ implies the existence of a rubber $r=f(\underline{H}^{i_1}_{j_1})$ joining a pair of vertical boundaries of the rectangles $V^{k_2}_{l_2}$ and $V^{k_1}_{l^1}$ that correspond to the image  of the upper boundary of $H^{i_1}_{j_1}$ inside $V^{k_1}_{l^1}$ and the image of the inferior boundary of $H^{i_1}_{j_1+1}$ inside $V^{k_2}_{l^2}$.

In the situation when $\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)$ we can assume bot of them are positive (or negative, but the reasoning is the same). 

The condition: $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ implies that the rubber $r'=f(\underline{H}^{i_2}_{j_2})$ joints the stable boundary of $V^{k_2}_{l_2}$ that is the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ with the stable boundary $V^{k_1}_{l^1}$ that is the image  by $f$ of the upper boundary of $H^{i_2}_{j_2}$. 

Like $\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)$ this implies that $r$ joins the upper boundary of $V^{k_1}_{l^1}$ with the inferior boundary of $V^{k_2}_{l_2}$, even more like $$\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)=1$$
the $r'$ joins the upper boundary of $V^{k_1}_{l^2}$ (that is the image of the upper boundary of $H^{i_2}_{j_2}$) with the inferior boundary of $V^{k_2}_{l_1}$.
Like $l_1<l_2$ and $l^1<l^2$ the fist combinatorial condition implies that $\cR$ have a topological obstruction of type $(2)$.

Now if  $\rho_T(i_2,j_2)= (k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$, and 
$$\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)=-1$$,
The rubber rubber $r'$ have stable boundary in the upper boundary of $V^{k_1}_{l_2}$ as this correspond to the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ with the  inferior boundary of $V^{k_2}_{l_1}$ that correspond to the image by $f$ of the upper boundary of $H^{i_2}_{j_2}$. Therefore we have a type $(2)$ obstruction.

Consider now that $\epsilon_T(i_1,j_1)=-\epsilon_T(i_1,j_1+1)$. Too fix ideas  $\epsilon_T(i_1,j_1)=1$ and $\epsilon_T(i_1,j_1+1)=-1$. This means that $r$ joins the upper boundary of $V^{k_1}_{l^1}$ (that is the image by $f$ of the upper boundary of $H^{i_0}_{j_0}$)
with the upper boundary of $V^{k_2}_{l_2}$ (that correspond to the image by $f$ of the inferior boundary of $H^{i_1}_{j_2+1}$ ).

 The condition  $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ of the point $(2)$ in the definition together with:
 $$
\epsilon_T(i_2,j_2)=1 \text{ and  } \epsilon_T(i_2,j_2+1)=-1.
$$
implies that $r'$ joints the superior boundary of $V^{k_1}_{l^2}$ that is the image by $f$ of the upper boundary of $H^{i_1}_{j_1}$, with the upper boundary of $V^{k_2}_{l_2}$ that is the image by $f$ of the inferior boundary of $H^{i_1}_{j_1+1}$. Similarly we have the obstruction of type $(2)$ in the Markov partition.

Finally if  $\epsilon_T(i_1,j_1)=1$ and $\epsilon_T(i_1,j_1+1)=-1$ but now $\rho_T(i_2,j_2)=(k_2,l_1), \rho_T(i_2,j_2+1)=(k_1,l^2)$ and 
$$\epsilon_T(i_2,j_2)=1 \text{ and  } \epsilon_T(i_2,j_2+1)=-1.$$

we can deduce that $r'$ joints the upper boundary of $V^{k_1}_{l^2}$ that is the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ and the upper boundary of $V^{k_2}_{l_1}$ that is the image by $f$ of the upper boundary of $H^{i_2}_{j_2}$. Once again we get a type two obstruction.

If the Markov partition $\cR$ have the type $(2)$ the ribbons $r$ and $r'$ determine the horizontal sub-rectangles determined by $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)$  and we can fix the condition 	$\rho_T(i_1,j_1)=(k_1,l^1)$ and $\rho_T(i_1,j^1+1)=(k_2,l_2)$ to indicate that $r$ joints such rectangles. The condition $(1)$ reflex the case when the two rectangles $R_{k_1}$ and $R_{k_2}$ have cohered orientation and the other case when they have inverse orientation. In any case, we need to remember that $r$ joint the image of the upper boundary of $H^{i_0}_{j_0}$ with the image of the inferior boundary of $H^{i_0}_{j_0}$. The four conditions enunciated are all the possible case when the ribbon $r'$ have stable boundaries in the same stables boundaries components of $\cR$ than $r$.

\end{proof}




\begin{defi}\label{Defi: Type 3 combinatoric}
A geometric type $T$ satisfies the \emph{combinatorial condition} of type-$(3)$ if there exist indices and conditions described as follows:
\begin{itemize}
\item Three numbers $k_1,k_2,k_3\in \{1,\cdots,n\}$ such that, for $\sigma=1,2$ or $3$:
\begin{eqnarray}
\Phi(k_{\sigma},1)=(k_{\sigma},l_{\sigma},\epsilon(k_{\sigma},1)=1) \text{ or }\\
\Phi(k_{\sigma},h_{k_{\sigma}})=(k_{\sigma},l_{\sigma},\epsilon(k_{\sigma},h_{\sigma})=1).
\end{eqnarray}
where $l_1\in \{1,\cdots,v_{k_{\sigma}}\}$.
\item A couple of numbers $1 \leq l_1'<l_1''<v_{k_1}$ such that: either $l_1'<l_1''<l_1$ or $l_1<l_1'<l_1''<l_1''$.
\item For $\sigma=2,3$, a number $l_{\sigma}'$ with $1\leq l_{\sigma}'\leq v_{k_{\sigma}}$, and
\item A pair of elements in $\cH$, $(i_2,j_2)$ and $(i_3,j_3)$.
\end{itemize} 
All of them complying with the following:
\begin{eqnarray}
\Phi(i_2,j_2)=(k_1,l_1',\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l_2',\epsilon(i_2,j_2+1)), \text{ or well }\\
\Phi(i_2,j_2+1)=(k_1,l_1',\epsilon(i_2,j_2+1)) \text{ and } \Phi(i_2,j_2)=(k_2,l_2',\epsilon(i_2,j_2)).
\end{eqnarray}
and at the same time:
\begin{eqnarray}
\Phi(i_3,j_3)=(k_1,l_1'',\epsilon(i_3,j_3)) \text{ and } \Phi(i_3,j_3+1)=(k_3,l_3',\epsilon(i_3,j_3+1)), \text{ or well }\\
\Phi(i_3,j_3+1)=(k_1,l_1'',\epsilon(i_3,j_3+1)) \text{ and } \Phi(i_3,j_3)=(k_3,l_3',\epsilon(i_3,j_3))
\end{eqnarray}
A geometric type $T$ has the \emph{combinatorial obstruction} of type-$(3)$ if there exists an $m\in \NN$ such that $T^m$ satisfies the combinatorial condition of type-$(3)$.
\end{defi}


\begin{lemm}\label{Lemm: Equiv com and top type 3}
A geometric type have $T$ has the combinatorial condition of type $(3)$ if and only if the Markov partition $\cR_0$ hs the topological obstruction  of type-$(3)$ on $\cR_1$. 
\end{lemm}


\subsubsection{The impasse property.}

Finally we proceed to formulate the impasse condition in terms of the geometric type.


\begin{defi}\label{Defi: Impasse combinatoric}
 Let $T$ be an abstract geometric type of finite genus. If $T=(m,\{(h_i,v_i)\}_{i=1}^n, \phi:(\rho,\epsilon):\cH\rightarrow \cV\times\{-1,1\})$, then $T$ has the \emph{impasse property} if there exist $(i,j),(i,j+1)\in \cH$ such that one of the following conditions holds:
 
\begin{eqnarray}
(\rho,\epsilon)(i,j)=(k,l,\epsilon(i,j)) \text{ and } (\rho,\epsilon)(i,j+1)=(k,l+1,-\epsilon(i,j)), \text{ or }\\
(\rho,\epsilon)(i,j)=(k,l+1,\epsilon(i,j)) \text{ and } (\rho,\epsilon)(i,j+1)=(k,l,-\epsilon(i,j)).
\end{eqnarray}
A geometric type $T$ has a \emph{combinatorial impasse} if there exists $m \in \mathbb{N}$ such that $T^m$ has the impasse property.
\end{defi}


Unlike the first three obstructions, where a ribbon is determined by two horizontal sub-rectangles and their respective indices $(i,j),(i,j+1)\in \mathcal{H}$, a topological impasse is defined in terms of a disjoint disk of $K$ and two arcs. Proving the equivalence between the topological and combinatorial formulations just given is a more subtle task, and we address it in the final part of this subsection.

\begin{theo}\label{Theo: Geometric and combinatoric are equivalent}
Let $T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi)$  be a geometric type of finite genus. Let $f: S \rightarrow S$ be a surface Smale diffeomorphism, and let $K$ be a saddle-type basic piece of $f$ that has a Markov partition of geometric type $T$. The following conditions are equivalent:

\begin{itemize}
\item[i)] The basic piece $K$ has a topological impasse.
\item[ii)] The geometric type $T^{2n+1}$ has the impasse property.
\item[iii)] The geometric type $T$ has a combinatorial impasse.
\end{itemize}
\end{theo}


\begin{proof}
 \textbf{ i) implies ii):} Let  $\cR=\{R_i\}_{i=1}n$ be a Markov partition of $K$ of geometric type $T$, and let $\overset{o}{D}$ be a topological impasse with $\alpha$ as the $s$-arc and $\beta$ as the $u$-arc, whose union forms the boundary of $D$.

 \begin{lemm}\label{Lemm: impasse disjoin int Markov partition}
The impasse is disjoint from the interior of the Markov partition, i.e.
$$
\overset{o}{D}\cap \cup_{i=1}^n \overset{o}{R_i}=\emptyset.
$$
Moreover, the intersection $\{k_1,k_2\}=\alpha\cap \beta$ is not contained in the interior of the Markov partition.
 \end{lemm}
 
\begin{proof}
Suppose that $\overset{o}{D}\cap \overset{o}{R_i}\neq \emptyset$. Let $\{k_1,k_2\}:=\alpha\cap \beta$ be the extreme points of the $s,u$-arcs on the boundary of $D$. There exists an unstable segment $J$ of $R_i$ such that $k_1\in J$. Moreover, $k_2$ is either in the interior of $J$ or on the stable boundary of $R_i$.  The second case is not possible since $k_2$ would be isolated from $K$ both from above and below, and there are no double $s$-boundary points in $K$. 


By similar arguments, we can conclude that $k_1$ and $k_2$ are in $\overset{o}{R_i}$. However, this leads to a contradiction as there would be a horizontal segment $I$ and a vertical segment $J$ of $R_i$ intersecting at two points in the interior of $R_i$ (namely $k_1$ and $k_2$). This is not possible, thus contradicting our assumption. Hence, $\overset{o}{D}$ is disjoint from the interior of $R_i$.

\end{proof}



If $\overset{o}{D}$ is an impasse, then $f^z(\overset{o}{D})$ is also an impasse for all integers $z \in \ZZ$. In the following lemma, we will construct a "well-suited" impasse that will make it easier for us to prove the first implication.

\begin{lemm}\label{Lemm: well suit impasse}
If $K$ has an impasse, then there exists another impasse $D'$ of $K$ such that the $s$-arc $\alpha'$ and the $u$-arc $\beta'$ on the boundary of $D'$ satisfy the following conditions:

\begin{itemize}
\item[i)]  $\beta'$ is in the interior of the unstable boundary of the Markov partition,  $\beta' \subset \overset{o}{\partial^u  \cR}$,
\item[ii)] $f(\beta')$ is not a subset of the unstable boundary of the Markov partition,  $\partial^u\overset{o}{\cR}= \overset{o}{\partial^u  \cR}$.
\item[iii)] $f^{2n+1}(\alpha)\subset \overset{o}{\partial^s \cR}$, where $n$ is the number of rectangles in the Markov partition.
\end{itemize}
\end{lemm}
 
 \begin{proof}
Let $D$ be an impasse of $K$ with $\alpha$ and $\beta$ as its boundary arcs. Let $\{k_1,k_2\}:=\alpha \cap \beta \subset K$ be the extreme points of these arcs. If $k_1$ is a periodic point, then there exists a positive iteration of $k_2$ that intersects $\alpha$ in its interior. However, this is not possible since the interior of $\alpha$ is disjoint from $K$. Therefore, we deduce that $k_1$ and $k_2$ are on the same stable separatrice of a periodic $s$-boundary point, and they are not periodic points themselves. Similarly, $k_1$ and $k_2$ are on the same unstable separatrice of a $u$-boundary point, but they are not periodic.

Since the negative orbit of $k_1$ converges to a periodic point $p_1$ on the stable boundary of the Markov partition, the negative orbit of $k_1$ approaches $p_1$ through points contained in the boundary of the Markov partition. Therefore, there exists $m \in \NN$ such that $f^{-m}(k_1)\in \overset{o}{\partial^u \cR}$.  We claim that if $f^{-m}(k_1)\in \overset{o}{\partial^u_{\epsilon}R_i}$, then $f^{-m}(k_2)$ is in the interior of the same unstable boundary component as $f^{-m}(k_1)$, i.e., $f^{-m}(k_2)\in \overset{o}{\partial^u_{\epsilon}R_i}$.

Indeed, since $f^{-m}(k_1)$ and $f^{-m}(k_2)$ are the boundary points of the $u$-arc $f^{-m}(\beta)$, there are no points of $K$ between them. The point $f^{-m}(k_1)$ lies in the interior of $\partial^u_{\epsilon} R_i$, which means that $f^{-m}(\beta)$ intersects the interior of this stable boundary component. This implies that $f^{-m}(k_2)$ is either an extreme point of $\partial^u_{\epsilon} R_i$ or lies in its interior, i.e., $f^{-m}(k_2) \in \overset{o}{\partial^u_{\epsilon}R_i}$.

If $f^{-m}(k_2)$ were an extreme point of $\partial^u_{\epsilon} R_i$, such an extreme point would not be surrounded by elements of $K$ on either side. This is because on one side we have the $u$-arc $f^{-m}(\beta)$, and on the other side it is on the unstable boundary of a rectangle in the Markov partition. However, this is not possible since $K$ has no double $s$-boundary points. Therefore, we conclude that $f^{-m}(k_2) \in \overset{o}{\partial^u_{\epsilon}R_i}$, as we claimed.


Now let us consider the impasse $D' = f^{-m}(D)$ instead of $D$. We will still use $\alpha$ and $\beta$ to denote the $s$-arc and $u$-arc on the boundary of $D$, but we assume that $\beta \subset \overset{o}{\partial^u \cR}$. Due to the uniform expansion along the unstable leaves, we know that there exists $m \in \NN$ such that $f^m(\beta) \subset \overset{o}{R_i}$, but $f^{m+1}(\beta)$  is no longer contain in  the unstable boundary of the Markov partition. Let us define $D' = f^{m}(D)$ with boundary arcs $\alpha'$ and $\beta'$. This impasse satisfies items $i)$ and $ii)$ of our lemma, since $\beta'$ is contained in the interior of $\overset{o}{\partial^u \cR}$ and $f(\beta')$ is not a subset of $\partial^u \overset{o}{\cR} = \overset{o}{\partial^u \cR}$.


In view of Lemma \ref{Lemm: impasse disjoin int Markov partition}, the points $f(k_1)$ and $f(k_2)$ are not in the interior of the Markov partition. We conclude that $f(k_1)$ and $f(k_2)$ belong to $\partial^s \cR$ because both are on the boundary of $\cR$ but not inside the unstable boundary. By the invariance of the stable boundary of $\cR$ under positive iterations of $f$ and the Pigeonhole principle applied to the $2n$ components of stable boundaries of the Markov partition, we know that $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ lie on periodic stable boundaries of the Markov partition. Moreover, $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ lie on the same stable separatrice, and on each separatrice, there is a single stable boundary component of $\cR$ that is periodic (even though they are all pre-periodic). This implies that $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ are in $\overset{o}{\partial^s_{\epsilon}R_j}$ for a single stable boundary component of the rectangle $R_j$. This proves item $iii)$ of our lemma.

\end{proof}



With the simplification of  Lemma \ref{Lemm: well suit impasse} we deduce that $\beta\subset \partial^u R_i$ and $f^{2n+1}(\alpha)\subset \partial^s R_k$. 

Let us consider the partition $\cR$ viewed as a Markov partition of $f^{2n+1}$. We claim that $\beta$ is an arc joining two consecutive sub-rectangles of $(\cR,f^{2n+1})$, denoted as $H^i_j$ and $H^{i}_{j+1}$. In effect, $\beta$ is a $u$-arc joining two consecutive rectangles or is properly contained in a single sub-rectangle $H$ of $(\cR,f^{2n+1})$. This is because the stable boundaries of $H$ are not isolated from $K$ within $H$, as would be the case if the ends of $\beta$ were on the stable boundary of $H$. Therefore, the only possibility is that $\beta$ is properly contained in a rectangle $H$. In this case, $f^{2n+1}(H)$ is a vertical sub-rectangle of $R_i$ containing $f^{2n+1}(\beta)$ as a proper interval. However, the endpoints of $f^{2n+1}(\alpha)$, which coincide with the endpoints of $f^{2n+1}(\beta)$, are not in the interior of the stable boundary of $R_k$, which contradicts the hypothesis. Thus, we conclude that $\beta$ joins two consecutive sub-rectangles.


Let $H^i_{j}$ and $H^i_{j+1}$ be the consecutive rectangles joined by $\beta$. Suppose that $f^{2n+1}(H^i_j)=V^k_{l}$ with the change of vertical orientation encoded by $\epsilon_{T^{2n+1}}(i,j)$ and $f^{2n+1}(H^i_{j+1})=V^k_{l'}$ with the change in the vertical orientation encoded by $\epsilon_{T^{2n+1}}(i,j+1)$. Between $V^k_{l}$ and $V^k_{l'}$ there are no points of $K$ because the $s$-arc $f^{2n+1}(\alpha)$ joins them in the horizontal direction, this implies that $l'\in \{l+1,l-1\}$. The vertical orientation of $\beta$ is the same as $H^i_j$ and $H^i_{j+1}$, furthermore $f^{2n+1}(\beta)$ joins the horizontal sides of the rectangles $V^k_{l}$ and $V^k_{l'}$ which are on the same stable boundary component of $R_k$,  this implies that the vertical orientation of $f(H^i_j)$ is the inverse of the orientation on $f(H^i_{j+1})$ within $R_k$ (to visualize this it suffices to follow the segment $f^{2n+1}(\beta)$ with a fixed orientation), thus $\epsilon_{T^{2n+1}}(i,j)=-\epsilon_{2n+1}(i,j')$.


The geometric type of the Markov partition $\cR$ for the map $f^{2n+1}$ is $T^{2n+1}$. Our construction implies that $T^{2n+1}$ has the impasse property. With this, we conclude the first implication of the theorem..


 \textbf{ ii) implies iii):} The geometric type $T^{2n+1}$ has the impasse property, which implies that $T$ has a combinatorial impasse.
 

\textbf{ iii) implies i):} Suppose $T^m$ has the impasse property. Let $H^i_j$ and $H^i_{j+1}$ be consecutive horizontal sub-rectangles in the Markov partition $\cR$ for the map $f^{m}$, as given by the impasse property. This condition implies that if $f^{2n+1}(H^i_j)=V^k_{l}$ and $f^{2n+1}(H^i_{j+1})=V^k_{l'}$, then $l$ and $l'$ are consecutive and have inverse vertical orientations.


The stable segments of on the stable boundary of $R_k$ between $V^k_{l}$ and $V^k_{l'}$ do not contain elements of the maximal invariant set of $f^m\vert_{\cR }$, since they are consecutive sub-rectangles of the partition $\cR$ seen as a Markov partition of $f^m$. In fact they do not contain elements of $K$ since $K=f^m(K)$ and therefore those segments are $s$-arcs of $f$. Furthermore, the image by $f^{m}$ of the two arcs $u$ on the boundary  of $R_i$ that join $H^i_j$ and $H^i_{j+1}$ are $u$-arcs of $f$. Between the two pairs of arcs there is an $s$-arc $\alpha$ and a $u$-arc $\beta$ such that they intersect each other only at their ends. We affirm that $\alpha$ and $\beta$ delimit a disk $D$ with a disjoint interior of $K$.


Suppose that $\gamma:=\alpha \cup \beta$ does not bound a disk. This means that $\gamma$ is not homotopically trivial, and neither are its iterations $\{f^m(\gamma)\}{m=1}^{\infty}$. In fact, since the stable segments of such curves lie in the stable manifold of a periodic point, there exists a $k\in \NN$ such that $\{f^{mk\}(\gamma)}{m=1}^{\infty}$ is a set of disjoint curves. We will argue that two of these curves are not homotopic, leading to a contradiction with the fact that the surface $S$ where the basic piece is contained has finite genus.

\begin{lemm}\label{Lemma: gamma not homotopic imagen}
The curve $\gamma$ is not homotopic to any other curve $f^{2mk}(\gamma)$ for $k\in \mathbb{N}$.
\end{lemm}


\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{Preliminares/Imagenes/Anillo.png}
	\caption{ The Annulus}
	\label{Fig: The annulus}
\end{figure}


\begin{proof}
Suppose $\gamma$ and $f^{m}(\gamma)$ are homotopic, which means they bound a topological annulus $\AA$ in $S$. Let us endow the boundary of $\AA$ with the clockwise orientation, and assume that $\gamma$ represents the interior boundary of $\AA$, while $f^m(\gamma)$ represents the exterior boundary.

Then, under the map $f^m$, a small sub-annulus $\mathcal{A}'$ of $\mathcal{A}$, which has $\gamma$ as one of its boundary components, is mapped to another annulus $f^m(\mathcal{A}')$, where $f^m(\gamma)$ serves as a boundary component. Here is the key point: if $f^m(\gamma)$ preserves the clockwise orientation, we can make $\mathcal{A}'$ small enough so that the interior of $f^m(\mathcal{A}')$ is disjoint from $\mathcal{A}$.


Suppose $f^m$ reverses the clockwise orientation of $\gamma$. We emphasize that $\gamma$ and $f^{2m}(\gamma)$ are still homotopic and bound an annulus $\mathcal{A}$. However, in this case, $f^{2m}$ preserves the clockwise orientation of the inner boundary. Hence, there exists a small sub-annulus $\mathcal{A}'$ of $\mathcal{A}$ that is bounded by $\gamma$, and the interior of $f^{2m}(\mathcal{A}')$ is disjoint from $\mathcal{A}$. Therefore, we can assume that $\gamma$ and $f^{2km}(\gamma)$ satisfy this property.

Suppose that $\gamma$ is saturated by the hyperbolic set $K$ in the interior direction of $\AA$, and therefore, it is isolated from $K$ in the exterior direction of $\AA$. Then $f^{2km}(\gamma)$ is isolated from $K$ in the interior direction of $\AA$ and saturated by $K$ in the exterior direction of $\AA$. In particular, there exists $x\in K \cap (S \setminus \AA)$.
 
Since ${k_1, k_2}$ and ${f^m(k_1), f^m(k_2)}$ are not periodic points, they do not have free separatrices. Moreover, $k_1$ and $k_2$ lie on the same separatrice. Without loss of generality, let's assume that $k_1$ has a stable separatrice $I$ that does not connect it to a periodic point. The separatrice $I$ cannot remain entirely inside $\AA$ because there exists a point $x \in K$ outside of $\AA$. Non-free separatrices of points $y \in K$ that do not connect $y$ to a periodic point are dense in $K$, so $I$ needs to approach $x$ arbitrarily closely. The boundary of $\AA$ is the union of four arcs, which means that the separatrice $I$ cannot intersect them in their interiors. Therefore, the possible scenarios are as follows:

 \begin{itemize}
\item The intersection point is $k_2$, which is impossible since it would imply that $I$ is inside a closed leaf of $W^s(K)$,
\item The other point is $f^m(k_1)$ or $f^m(k_2)$. This is not possible because in that case, $I$ would need to be contained in the separatrice of $f^m(k_1)$ (or $f^m(k_2)$), which is not the same as the $s$-arc in $f^{2km}(\gamma)$. But this separatrice points towards the exterior of $\AA$
 \end{itemize}
 
So, $I$ couldn't intersect either $f^m(\gamma)$ or $\gamma$. We conclude that $I$ is a subset of $\AA$, which is a contradiction. This ends our proof.
 
\end{proof}

Then, if $\gamma$ is not null-homotopic, we could find an infinite amount of disjoint and non-isotopic curves (See \cite[Lemma 3.2]{juvan1996systems}), which is a contradiction with the finite genus of the surface $S$. It follows that $\gamma$ bounds a disk.


\begin{coro}\label{key}
	
	The disk bounded by $\gamma$ doesn't intersect $K$.
\end{coro}

\begin{proof}
If there exists $x \in K \cap \overset{o}{D}$, then $x$ has at least one non-free stable separatrice $I$. Such a separatrice is not confined within $D$ because there exist points in $K$ that are not in $D$ (they are those on the other side of the $s$-arc $\alpha$ on the boundary of $D)$. Additionally, $I$ is dense in $K$. Therefore, $I$ must intersect the $u$-arc $\beta$ on the boundary of $D$. However, the separatrice $I$ does not intersect the extreme points $\{k_1,k_2\}=\alpha \cap \beta$ because no local separatrices of them intersect the interior of $D$. This leads to a contradiction. Hence, $K \cap \overset{o}{D} = \emptyset$.
\end{proof}



This implies that $D$ is an impasse for $f$.



\end{proof}

\subsection{Algorithmic Determination of Finite Genus and Impasse }\label{Sub-sec: algoritm finite genus}


The objective is to prove the following proposition that will serve as the key element in determining, algorithmically and in finite time, whether a geometric type belongs to the pseudo-Anosov class or not. In the future, we will derive the property of double boundaries from the fact that the incidence matrix of a geometric type in the pseudo-Anosov class is mixing. Therefore, we formulate this property as the first one to be verified.

\begin{prop}\label{Prop: mixing+genus+impase is algorithm}
	Given any abstract geometric type $T=(n\{(h_i,v_i),\},\Phi)$, there exists a finite algorithm that can determine whether $T$ satisfies the following properties:
	\begin{enumerate}
		\item The incidence matrix of $T$, $A(T)$ is mixing. 
		\item The genus of $T$ is finite.
		\item  $T$ exhibits an impasse.
	\end{enumerate}
	Furthermore, the number of iterations of $T$ required by the algorithm to determine these properties is upper bounded by $6n$, where $n$ represents the size of $T$.
\end{prop}



\begin{proof}
	
	We have formulated specific conditions on the combinatorics of $T$ to determine whether $T^n$ has an impasse or one of the three obstructions to have finite genus. Furthermore, according to Theorem \ref{Theo: finite type iff non-obstruction}, determining whether or not $T$ has finite genus requires computing at most $T^{6n}$. To determine whether $T$ has an impasse, Theorem \ref{Theo: Geometric and combinatoric are equivalent} states that it is necessary to compute at most $T^{2n+1}$. Since $n\geq1$, it is clear that $2n+1<6n$, which provides the upper bound we claim in the proposition. Proposition \ref{Prop: algorithm iterations type} asserts that the computation of $T^{6n}$ is algorithmic, thus confirming the existence of an algorithm to determine the finite genus and the presence of an impasse for $T$.
	
	
	
	
	We have left the mixing criterion for last. The following lemma is the basis for the upper bound on the number of iterations to verify the mixing of the incidence matrix.
	
	\begin{prop}\label{Prop: bound positive incidence matriz }
		If $A$ is a non-negative mixing matrix of size $n \times n$, then $A^n$ is positive definite.
	\end{prop}
	
	\begin{proof}
		
		Consider the directed graph $\mathcal{G}$ with $n$ vertices corresponding to the matrix $A$. In this graph, there is an edge pointing from vertex $v_i$ to vertex $v_j$ if and only if $a_{ij} > 0$ in the matrix $A$. Since $A$ is mixing, it means that there is always a path from any vertex $v_i$ to any other vertex $v_j$ in the graph $\mathcal{G}$.
		
		To prove our Lemma, it is sufficient to demonstrate that there exists a path of length less than or equal to $n$ between any two vertices in the graph.
		
		
		
		Consider a path $\gamma = [v_{i(1)}, \cdots, v_{i(m)}]$ from $v_i = v_{i(1)}$ to $v_j = v_{i(m)}$ in the graph $\mathcal{G}$. Let $\gamma$ have $m$ vertices and be of minimum length among all paths connecting these vertices.
		
		If any two vertices of the path $\gamma$ are equal, it implies the existence of a cycle within $\gamma$. We can eliminate this cycle and obtain a new path $\gamma'$ from $v_i$ to $v_j$ with a shorter length than $\gamma$. This contradicts the assumption that $\gamma$ has the minimum length. Hence, all vertices in $\gamma$ must be distinct.
		
		Therefore, the length of $\gamma$ is necessarily less than or equal to $n$, since there are only $n$ distinct vertices in the graph.
	\end{proof}
	
	
	If $T$ is in the pseudo-Anosov class, we have $A^n(T) = A(T^n)$. According to the previous Lemma, if $A(T)$ is a non-negative matrix, then $A(T^n)$ is positive definite. This implies that $A(T^n)$ is mixing and does not have double boundaries. Therefore, for a given geometric type $T$ with $A(T)$ being a non-negative matrix, the positivity of $A(T^n)$ is equivalent to its mixing property, which in turn implies the absence of double boundaries.
	
	\begin{coro}\label{Coro: algoritmic mixing}
		Given a geometric type $T$, if $A(T^n)$ is not positive definite, then $T$ is not in the pseudo-Anosov class.
	\end{coro}
	
	Clearly, we only need to iterate $T$ $n$ times, and the upper bound given in the proposition remains valid. 
	This concludes our proof.
\end{proof}

==> TypeConjugacy/SubEulerandType.tex <==
\section{The Euler characteristic and the geometric type}\label{Sec: euler characteristic}

 For now lets point some result of independent importance. Previously we didn't demand a  knowledge of the surface $S$ where of pseudo-Anosov homeomorphism $f$ acts, instead, by assuming that $S$ accepts a pseudo-Anosov homeomorphism of geometric type $T$ we  could deduce the Euler characteristic of of $S$. The core of our analysis is the \emph{Euler-Poincare formula}:
 
 \begin{prop}\label{Prop; Euler Poincare formula}[Euler-Poincare formula]
 	Let $S$ be a closed surface with a singular foliation $\cF$. Let $P_s$ be the number of prongs at a singular point $s$. Then
 	$$
 	2\chi(S)=\sum_{s\in \text{Sing}(\cF)}(2-P_s).
 	$$
 \end{prop}
 

  Let $f:S\rightarrow S$ be a pseudo-Anosov homeomorphism with measured foliations $(\cF^s,\mu^s)$ and $(\cF^u,\mu^u)$ in this section we assume that:
\begin{itemize}
\item $S$ is a closed surface with finite set of marked points $P\subset S$.
\item $f:S\rightarrow S$ is a pseudo-Anosov homeomorphism with all their spines contained in $P$.
\item The set of singularities of $f$ is denoted as Sing$(f)$.
\end{itemize}

\subsection{The pictorial algorithm}

Let $T$ be a geometric type in the pseudo Anosov class, we are going to see in  Chapter \ref{Chapter: Realization}  that $T$ admits  a realization by disjoint rectangles, $(\cR'=\{R_i\}_{i=1}^{n},\Phi')$. This result is independent of this section, so we are going to assume the existence of such family.
Let $0\leq m\leq 4n'$ a natural number such that every periodic boundary point of $\Phi'$  and every separatrice in the boundary of the rectangles in $\cR'$ are fixed by $\phi$. 


Let $f:S\rightarrow S$ be a pseudo-Anosov homeomorphism with a Markov partition of geometric type $T$, then  $T^m$ is the geometric type of a Markov partition of $f^m:S \rightarrow S $  and then  is in the pseudo-Anosov class, therefore $T^m$  and admits a realization by disjoint rectangles $(\cR=\{R_i\}_{i=1}^n,\phi)$. We should use this realization to calculate the genus of $S$.


Let $p\in R_i$ a fixed stable boundary point and be $I\subset\partial^s R_i$ be a stable separatrice of $p$, we could deduce what other separatrice $I'$ is identify with $I$ in the next manner.

Let ${V^i_l}_{l=1}^L$ the set of vertical sub-rectangles of $R_i$ which have an stable boundary intersecting whose interior intersect $I$. Suppose that for all $l$ :
$$
V^i_l=\Phi(H^{i(l)}_{j(l)}).
$$ 

The stable separatrice $I$ is necessarily identify with another separatrice $I'$, then there is at lest one $l\in \{1,\cdots, L\}$ such that: there exist $j'\in \{1,\cdots, v_{i(l)}\}\setminus\{j(l)\}$ such that if:
$$
\Phi^(H^{i(l)})_j'=V^{i'}_{l'}
$$
 and,  if the interior of (upper) inferior boundary $I_-$ of $H^{i(l)}_{j(l)}$ is such that $\Phi(\overset{0}{I_-})\cap  \overset{o}{I}\neq \emptyset $ then the interior of the (inferior) upper boundary $I_+$  of $H^{i(l)})_j'$ satisfy that $\phi(\overset{o}{I_+})\cap I'\neq \emptyset$. This procedure determines unequivocally the separatrices that are identified. This construction allows us to know how many stable separatrices the point $p$ has, i.e. we have been able to calculate $P_p$. This graphical description permits to calculate the Euler characteristic using a draw of the rectangles, this is why we call it pictorial algorithm.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{TypeConjugacy/Imagenes/sepindetify.pdf}
	\caption{Two stable segments.}
	\label{Fig: Two segments}
\end{figure}

\subsection{The symbolic algorithm.}

Let $T$ a geometric type in the pseudo-Anosov class, let $(\Sigma_T,\sigma_T)$ it combinatorial model, be  $\cR={R_i}_{i=1}^n$ a a Markov partition of $\Sigma_T$ of geometric type $T$. Let $\pi:\Sigma_A \rightarrow \Sigma_T$ the semi-conjugation. We recall some definitions and result of our previous section:
\begin{itemize}
 \item The set of $s,u$-periodic boundary points of $(\Sigma_A,\sigma)$ is calculated using the $s,u$-boundary generating function ( see ~ \ref{Defi: s-boundary generating funtion}). Even more, like we are looking for boundary periodic points, it period is at most $2n$, then it is enough to applied such function $2n$ times, for ever pair $i_0\in \{1,\cdots,n\}$ and $\epsilon_0=\pm 1$, which is finite set. We fix the notation:
 $$
 Per_{s,u}(A)=\{\underline{w}\in \Sigma_A: \underline{w} \text{ is a } s,u-\text{periodic boundary code } \}
 $$
 and 
 $$
  Per_{B}(A)= Per_{s}(A)\cup  Per_{u}(A).
 $$
 \item The set of $s,u$-periodic boundary points of $\Sigma_T$ is obtained by:
 $$
 Per_{s,u}(T)=Per_{s,u}(A)/\sim_T.
 $$
It calculation is algorithmic as $\sim_T$ is determined algorithmically.
 \item The function, $\pi:\sigma_A \rightarrow \Sigma_T$  is determine by $\sim_T$ and then it definition is algorithmic.
\end{itemize}


Let $[w]\in Per_B(T)$, suppose that $[w]$ have $k$-prongs, the set of admissible codes that project to $[w]$ is $\pi^{-1}([w])=\{\underline{w_j}\}_{j=1}^m$, every one of this codes is an \emph{sector code} of $[w]$, then $m\leq 2k$. If fact if $[w]$ is in the corner of every rectangle $R_i\subset \Sigma_T$ that contains $[w]$, $m=2k$. Then
$$
P_{[w]}=\frac{m}{2}.
$$
But suppose that $[w]$  is a $s$-boundary periodic point of $\sigma_T$ that is in the interior of the stable boundary of a rectangle $R_i$, then, there is two sector codes of $[w]$ that are equal, like the number of prong of $[w]$ is equal to $\frac{1}{2}$ of the amount of sector codes  of $k$ we could define the following function:
$$
a(\underline{w}) =
\begin{cases}
1 & \text{if } w\in Per_{s}(A)\cap Per_u(A)  \\
2 & \text{if } w\in Per_{s}(A)\setminus Per_u(A) \cup  Per_{u}(A)\setminus Per_s(A)  
\end{cases}
$$

and then we calculate $P_[w]$ as:
$$
\frac{1}{2}P_[w]= \sum_{\underline{w}\in \pi^{-1}([w])}a(\underline{w}).
$$


Once we have the previous information we could use Euler-Poincare formula to determine the Euler characteristic and we obtain the following result.



\begin{coro}\label{Coro: Algorithm to Euler characteritic}
Let $T$ be a geometric type in the pseudo-Anosov class, and let $f:S\rightarrow S$ be a generalized pseudo-Anosov homeomorphism with a geometric Markov partition of type $T$. There exists a finite algorithm that, given $T$, determines the number of $k$-prongs of $f$ (for every $k\geq 0$) and the Euler characteristic of $S$.
\end{coro}




